SPDZCoder: Combining Expert Knowledge with LLMs for Generating Privacy-Computing Code

Privacy computing receives increasing attention but writing privacy computing code remains challenging for developers due to limited library functions, necessitating function implementation from scratch, and data-oblivious requirement, contradicting intuitive thinking and usual practices of programmers. Automating the generation of privacy computing code with Large Language Models can streamline development effort and lower the barrier to using privacy computing frameworks. However, existing LLMs still encounter challenges in code translation for privacy-preserving computation, such as translating Python to MP-SPDZ, due to the scarcity of MP-SPDZ data required for effective pre-training or fine-tuning. Moreover, the lack of a benchmark further complicates the evaluation of translation quality. To address the limitations, this work proposes SPDZCoder, a rule-based framework that combines LLMs with expert knowledge for generating privacy-computing code without requiring additional training data. Specifically, SPDZCoder employ a rigorous procedure for collecting high-quality expert knowledge to represent the semantic-expressing differences between Python and MP-SPDZ, and to derive transformation rules for translating Python to MP-SPDZ based on these knowledge. Then, SPDZCoder progressively converts Python code into MP-SPDZ code using transformation rules in a three stage pipeline. To evaluate SPDZCoder, we manually constructed a benchmark dataset, SPDZEval, which comprises six data splits, each representing a distinct class of challenging tasks in MP-SPDZ implementation. Extensive experiments show that SPDZCoder achieves superior performance, significantly surpassing baselines in pass@1 and pass@2. Specifically, SPDZCoder attains an overall correctness of 85.94% and 92.01% in pass@1 and pass@2, respectively, whereas the best-performing baseline achieves 63.58% and 76.36%, respectively.

==> 05_Related_Work.tex <==
\section{Related Work}
% We discuss the most recent advances in LLMs, code translation approaches, and code generation benchmarks.
\subsection{Large Language Models}
% 通用大模型
General LLMs \cite{brownLanguageModelsAre2020a, chowdhery_palm_2022, touvron_llama_2023, touvron_llama_2023-1, claude3, openai_gpt-4_2023, gemini_team_gemini_2023, workshop_bloom_2023, jiang_mixtral_2024, glm2024chatglm, gpt-4o, deepseekai2024deepseekv3technicalreport} have rapidly advanced, demonstrating remarkable capabilities across diverse tasks. For example, GPT-4o has achieved state-of-the-art performance on code benchmarks such as HumanEval and MBPP. Similarly, DeepSeek-V3 achieves strong results in both natural language processing and code generation. 
Building on the success of LLMs, many research efforts have leveraged their capabilities to address specific challenges in software engineering, including code translation \cite{yangExploringUnleashingPower2024, macedoInterTransLeveragingTransitive2024a} (discussed below), fault localization \cite{yang_large_2024, li_fault_2022},~log analysis \cite{ma_knowlog_2024} and testing \cite{deng_large_2024}. % debugging \cite{huang_crashtranslator_2024}

% 代码大模型
Code LLMs are specialized large language models trained on multiple programming languages to support code understanding and generation.
A collection of studies focuses on the pre-training of code LLMs. DeepSeek-V2.5\cite{deepseekv2} integrates the strengths of DeepSeek-V2-Chat and DeepSeek-Coder-V2-Instruct, maintaining the conversational prowess while introducing advanced coding abilities. Qwen2.5-Coder\cite{hui2024qwen2} shows strong performance in code generation, repair, and reasoning across twelve benchmarks, achieving coding capabilities comparable to GPT-4o. Other pre-trained models include CodeGen\cite{nijkamp_codegen_2023}, CodeGeeX\cite{zheng_codegeex_2023}, StarCoder\cite{li_starcoder_2023}, and DeepSeek-Coder\cite{guo_deepseek-coder_2024}.
Another line of research focuses on fine-tuning code LLMs on curated code corpora to improve performance or adapt them to specific coding tasks, such as WizardCoder\cite{luo_wizardcoder_2023} and InstructCodeT5+~\cite{wang_codet5_2023}.

% 推理大模型
Reasoning LLMs enhance LLMs' capabilities in structured logical inference and decision-making, which are particularly crucial for tasks such as code generation, algorithm design, and mathematical problem-solving, as these tasks rely on step-by-step deduction. 
DeepSeek-R1 \cite{deepseekai2025deepseekr1incentivizingreasoningcapability} is trained via large-scale reinforcement learning (RL) without supervised fine-tuning (SFT) as the preliminary step, and it demonstrates remarkable reasoning capabilities, achieving performance comparable to OpenAI-o1 on reasoning tasks. Qwen-QwQ \cite{qwq-32b-preview} and OpenAI o1 \cite{openai-o1} also belong to RLLMs.
% OpenAI trained o1 \cite{openai-o1} model to learn to refine their thinking process, try different strategies, and recognize their mistakes, making it better at complex reasoning tasks. 

Pre-training or fine-tuning these LLMs requires massive or chain-of-thought code, which is largely absent in the field of privacy computing. In contrast, our approach leverages an in-context learning paradigm to enhance LLMs' effectiveness in code translation for privacy computing.



\subsection{Code Translation}
% transpilers
% learning-based
Most code translation approaches can be classified into transpiler approaches and learning-based approaches. In transpiler approaches \cite{noauthor_java_nodate, noauthor_c2rust_nodate, noauthor_cxgo_nodate}, which are restricted to syntactic modifications, researchers utilize program analysis techniques to covert code from one programming language to another. In the learning-based methods, which require preparing training data, people use Transformer-based structure to train a deep model to address either a specific code task or general code tasks. For instance, CodeBERT\cite{feng_codebert_2020} learns general-purpose representations of programming language and natural language in order to support downstream NL-PL applications such as natural language code search, code documentation generation, etc. In addition, CuBERT\cite{kanade_learning_2020}, GraphCodeBERT\cite{guo_graphcodebert_2021}, CodeT5\cite{wang_codet5_2021} and PLBART\cite{ahmad_unified_2021} also lie in this category. 

Beyond deep learning, LLMs are employed as backbone to perform code translation. For example, UniTrans \cite{yangExploringUnleashingPower2024} incorporates test cases to augment code translation and iteratively repair bugs for incorrectly translated programs prompted by test case execution results. 
InterTrans \cite{macedoInterTransLeveragingTransitive2024a} utilizes a planning algorithm (ToCT) to generate candidate translation paths, and leverages intermediate translations to enhance code translation. SPDZCoder also uses LLMs for code translation, but unlike UniTrans and InterTrans, our target programming language is not familiar to LLMs.



\subsection{Code Generation Benchmark}
Many works were proposed to benchmark the code generation ability of LLMs \cite{chen_evaluating_2021,liu_is_2023,yu_codereval_2024,athiwaratkunMultilingualEvaluationCode2022,lai2022ds1000naturalreliablebenchmark,cassanoMultiPLEScalablePolyglot2023,hendrycksapps2021,austin_program_2021,du_classeval_2023}. The Mostly Basic Programming Problems (MBPP) dataset \cite{austin_program_2021}, consisting of 974 programming tasks, measures the ability of LLMs to synthesize short Python programs from natural language descriptions. % MBPP consists of 974 programming tasks, designed to be solvable by entry-level programmers.
Human-eval\cite{chen_evaluating_2021} measures functional correctness for synthesizing programs from docstring.
%To overcome the limitation of test cases in quantity and quality for assessing the correctness of the generated code, 
Liu et al. proposed an enhanced code synthesis evaluation framework named EvalPlus\cite{liu_is_2023}, which augments HumanEval with large amounts of newly produced test-cases. Similar work also includes Multi-HumanEval \cite{athiwaratkunMultilingualEvaluationCode2022}.
More recently, parallel with ClassEval\cite{du_classeval_2023}, Yu et al. proposed CoderEval\cite{yu_codereval_2024} to evaluate the effectiveness of code LLMs in generating code beyond only standalone functions.% The benchmark curated 230 Python and 230 Java code generation tasks from popular real-world open-source projects and includes a self-contained execution platform to automatically assess the functional correctness of generated code.
% reference: A Survey on Large Language Models for Code
 There are also code generation benchmarks for specific purpose, \eg type prediction, fuzzing, code repair, unit test generation. For example, Mir \etal present ManyTypes4Py\cite{mir_manytypes4py_2021}, a large Python dataset for machine learning (ML)-based type inference. %, which contains a total of 5,382 Python projects with more than 869K type annotations and was split into training, validation and test sets by files.

SPDZEval differs from these datasets in terms of coding tasks, target programming languages, and input information. Additionally, it can assess whether data-oblivious codes can be effectively synthesized.
% SPDZEval differs from these datasets in coding task (code completion), target code language (MP-SPDZ) and input information (both programming language and natural language). 

==> images/img_rq3_backbone-experiment.tex <==
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.49\textwidth]{assets/RQ_3_radar.png} % scale=0.23
      \caption{Impact of Using Different LLMs in the Refactoring Stage on Translation Performance.}
      \label{fig:rq3_backbone-experiment}
\end{figure}

 % SPDZCoder references a non-existent MP-SPDZ Matrix method or leaves a placeholder function.
